Dynamics and Transport at the Threshold of Many-Body Localization

Many-body localized (MBL) systems do not approach thermal equilibrium under their intrinsic dynamics; MBL and conventional thermalizing systems form distinct dynamical phases of matter, separated by a phase transition at which equilibrium statistical mechanics breaks down. True MBL is known to occur only under certain stringent conditions for perfectly isolated one-dimensional systems, with Hamiltonians that have strictly short-range interactions and lack any continuous non-Abelian symmetries. However, in practice, even systems that are not strictly MBL can be nearly MBL, with equilibration rates that are far slower than their other intrinsic timescales; thus, anomalously slow relaxation occurs in a much broader class of systems than strict MBL. In this review we address transport and dynamics in such nearly-MBL systems from a unified perspective. Our discussion covers various classes of such systems: (i) disordered and quasiperiodic systems on the thermal side of the MBL-thermal transition; (ii) systems that are strongly disordered, but obstructed from localizing because of symmetry, interaction range, or dimensionality; (iii) multiple-component systems, in which some components would in isolation be MBL but others are not; and finally (iv) driven systems whose dynamics lead to exponentially slow rates of heating to infinite temperature. A theme common to many of these problems is that they can be understood in terms of approximately localized degrees of freedom coupled to a heat bath (or baths) consisting of thermal degrees of freedom; however, this putative bath is itself nontrivial, being either small or very slowly relaxing. We discuss anomalous transport, diverging relaxation times, and other signatures of the proximity to MBL in these systems. We also survey recent theoretical and numerical methods that have been applied to study dynamics on either side of the MBL transition.

==> acknowledgements.tex <==
\section{Acknowledgements}
We thank K.~Agarwal, I.~Bloch, P.~Bordia, E. Demler, P.T. Dumitrescu, A.J.~Friedman, A.~Goremykina, D.A.~Huse, V.~Khemani, M.~Knap, M.D.~Lukin, M.~M\"uller, R.~Nandkishore, A.C.~Potter, U.~Schneider, M.~Serbyn, R.~Vasseur and others for 
helpful discussions and collaborations on related work. S.G. acknowledges support from NSF DMR-1653271. S.A.P. acknowledges support from NSF Grant DMR-1455366 for previous research on some of the topics discussed in this review, and from EPSRC grant EP/S020527/1 as this review was completed. Both authors acknowledge the hospitality of the Kavli Institute for Theoretical Physics, which is supported by NSF Grant PHY-1748958, where some of this review was completed.

==> glossary.tex <==
\section{Glossary}

\begin{description}
\item[Area/volume law]
Succinct expression for the scaling of the (usually, von Neumann) entropy with the size of a subregion. Ground (highly excited) states of local Hamiltonians generically satisfy area (volume) laws for entanglement. MBL eigenstates satisfy area laws, while ETH dictates that eigenstates at finite energy density satisfy a volume law.
\item[Avalanche instability]
Nonperturbative instability of MBL systems in the presence of a thermal inclusion.
\item[ETH]
Eigenstate thermalization hypothesis. ETH posits that local expectation values of operators in any eigenstate of a many-body quantum chaotic system coincide with thermal expectation values at a temperature (and chemical potentials) set by the mean energy (and densities). 
\item[Frobenius inner product and Frobenius norm]
For two matrices $A$ and $B$, the Frobenius inner product $(A | B) = \mathrm{Tr}(A^\dagger B)$. The corresponding Frobenius norm is $\Vert A \Vert = \sqrt{(A | A)}$. 
\item[Griffiths effects/inclusions]
Rare regions in an inhomogeneous system in which the control parameter driving a phase transition is either unusually large or unusually small, so the system locally seems to be in the wrong phase.
\item[IPR]
Inverse participation ratio: defined for a normalized quantum state on a lattice as $\mathrm{IPR}_q = \sum_i |\psi_i|^{2q}$. When $q$ is not explicitly specified, it is assumed to be $2$. Generalizations can be defined for any normalized list.
\item[LIOM or l-bit]
A local integral of motion, i.e., a quasi-local operator $O$ that has a nonzero fraction of its support on a small, finite number of sites in the thermodynamic limit (i.e., has a finite inverse participation ratio in the Hilbert space of operators), and that \emph{exactly} commutes with the time-evolution operator.
\item[MBL]
Many-body localization (see main text). 
\item[MPO]
Matrix product operator. An MPO can be regarded as an operator written as a \emph{state} in the Hilbert space of operators, which is then compressed using MPS methods. One can equivalently regard an MPO as an operator that acts on the space of MPS's of a certain size. 
\item[MPS]
Matrix product state. A class of variational quantum states with low entanglement that are widely used in numerical simulations, because algorithms like TEBD rely on them.
\item[OTOC] 
Out-of-time-order correlator, defined as $\langle A(t) B(0) A(t) B(0) \rangle$ for arbitrary operators $A$ and $B$. Sometimes this acronym refers instead to the squared commutator, $\langle [A(t), B(0)]^2 \rangle$. While causal response functions measure the \emph{expectation value} of the commutator, the OTOC measures its variance. 
\item[perturbative resonance]
What happens in perturbation theory when the matrix element exceeds the energy denominator.
\item[R\'enyi entropy, Von Neumann entropy]
The $n$th R\'enyi entropy is defined as $S_n = (1 - n)^{-1} \mathrm{Tr}(\rho^n)$. The Von Neumann entropy is $S_1 \equiv \lim_{n \rightarrow 1} S_n = \mathrm{Tr} (\rho \ln \rho)$. Here, $\rho$ is a density matrix (typically the reduced density matrix when one is computing entanglement).
\item[RSRG, SDRG]
Real-space renormalization-group/strong-disorder renormalization group. A renormalization-group method that iteratively eliminates sites or bonds on a lattice and that is controlled for strong quenched randomness. Characterized by broad fixed-point distributions for various observables, as evinced by starkly congtrasting behavior of typical and disorder-averaged quantities.
\item[TEBD]
Time-evolving block decimation, a method for studying the dynamics of quantum states that are not too entangled, using a matrix-product representation. 

\end{description}

